MEC-enhanced Information Freshness for Safety-critical C-V2X Communications

Information freshness is a status update timeliness indicator of utmost importance to several real-time applications, such as connected and autonomous driving. The Ageof- Information (AoI) metric is widely considered as useful to quantify the information freshness of delivered messages to the involved entities. Recently, the advent of Multi-access Edge Computing (MEC) promises several performance benefits for Vehicular-to-Everything (V2X) communications, emphasizing on the experienced End-to-End (E2E) message delay. In this paper, we argue that, when it comes to safety-critical use cases, such as the one of Vulnerable Road User (VRU), additional metrics can be more insightful to evaluate and address scalability issues in dense urban environments. In particular, the impact of the packet inter-arrival time on the timeliness of VRU messages arriving at nearby vehicles can be directly assessed by exploiting the AoI metric. For that purpose, assuming a MEC-enabled multi-VRU system setting, we model the AoI and, by means of a performance comparison to the state-of-the-art network architecture based on numerical evaluations, we provide evidence of the information freshness and system scalability enhancements offered by MEC infrastructure deployment for different system parameter settings involving a large number of connected entities.

==> Inc_VRUM.tex <==
\definecolor{mycolor1}{rgb}{0.0, 0.0, 1.0}%\definecolor{ao}{rgb}
\definecolor{mycolor2}{rgb}{1.0, 0.01, 0.24}%\definecolor{americanrose}{rgb}
%
\begin{tikzpicture}
\pgfplotsset{
	width=2.4in,
	height=2.5in,
	scale only axis,
	xmin=10,
	xmax=100,
	xmajorgrids,
	ymajorgrids,
	legend style={legend columns =2,
		at={(0.78,0.95)},
		anchor=north east
	}
}
\begin{axis}[%
every outer y axis line/.append style={mycolor2},
every y tick label/.append style={font=\color{mycolor2}},
every y tick/.append style={mycolor2},
ymin=40,
ymax=240,
ylabel={\textcolor{mycolor2}{Avg. E2E latency [ms]}},
xlabel={VRU packet inter-arrival time ($T$) [ms]},
ylabel near ticks, yticklabel pos=right
]
\addlegendimage{legend columns=2, style={color=black, line width=2.0pt]}}
\addlegendentry{w/o MEC}
\addlegendimage{legend columns=2, style={color=black, dashed, line width=2.0pt]}}
\addlegendentry{w MEC}

\addplot [color=red, line width=2.0pt]
  table[row sep=crcr]{%
10	229.089515833047\\
20	183.261504933142\\
30	168.908096395577\\
40	162.990936012998\\
50	161.154239207361\\
60	156.747308374072\\
70	156.278454666592\\
80	151.822961274239\\
90	151.440094005067\\
100	150.051640455347\\
};

\addplot [color=red, dashed, line width=2.0pt]
  table[row sep=crcr]{%
10	114.9275792371\\
20	80.6620729486695\\
30	69.9974885441895\\
40	66.0923621694007\\
50	65.2045549258953\\
60	61.4201292262263\\
70	61.3918552286701\\
80	57.4473304700573\\
90	57.3644852973855\\
100	56.1311000353237\\
};

\draw[->, color=blue, line width=0.5mm](rel axis cs:0.5,0.73) -- (rel axis cs:0.32,0.48);
\draw[->, color=blue, line width=0.5mm](rel axis cs:0.5,0.22) -- (rel axis cs:0.32,0.42);
\node at (rel axis cs:0.2,0.45) {\textcolor{blue}{Peak AoI}};

\draw[->, color=red, line width=0.5mm](rel axis cs:0.8,0.55) -- (rel axis cs:0.72,0.48);
\draw[->, color=red, line width=0.5mm](rel axis cs:0.8,0.1) -- (rel axis cs:0.72,0.43);
\node at (rel axis cs:0.7,0.45) {\textcolor{red}{Avg. E2E latency}};

\end{axis}


\begin{axis}[%
every y tick label/.append style={font=\color{mycolor1}},
every y tick/.append style={mycolor1},
ymin=80,
ymax=260,
ylabel style={font=\color{mycolor1}},
ylabel={Peak AoI [ms]},
yticklabel pos=left,
xtick=\empty
]
\addplot [color=blue, line width=2.0pt]
  table[row sep=crcr]{%
10	239.089515833047\\
20	203.261504933142\\
30	198.908096395577\\
40	202.990936012998\\
50	211.154239207361\\
60	216.747308374072\\
70	226.278454666592\\
80	231.822961274239\\
90	241.440094005067\\
100	250.051640455347\\
};

\addplot [color=blue,dashed, line width=2.0pt]
  table[row sep=crcr]{%
10	124.9275792371\\
20	100.662072948669\\
30	99.9974885441895\\
40	106.092362169401\\
50	115.204554925895\\
60	121.420129226226\\
70	131.39185522867\\
80	137.447330470057\\
90	147.364485297385\\
100	156.131100035324\\
};

\end{axis}
\end{tikzpicture}%

==> Inc_VRUs.tex <==
\begin{tikzpicture}

\begin{axis}[%
width=2.8in,
height=2.45in,
scale only axis,
xmin=10,
xmax=290,
xlabel style={font=\color{white!15!black}},
xlabel={ Number of VRUs ($K$)},
ymin=100,
ymax=270.269876905179,
yminorticks=true,
ylabel style={font=\color{white!15!black}},
ylabel={Peak AoI [ms]},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.65,0.03)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=blue, line width=2.0pt, mark=o, mark options={solid, blue}]
  table[row sep=crcr]{%
10	197.976872671623\\
50	232.323851243008\\
90	245.646666103726\\
130	253.154418936708\\
170	258.69522421737\\
210	262.838769482113\\
250	266.552380800207\\
290	270.269876905179\\
};
\addlegendentry{w/o MEC}

\addplot [color=red, line width=2.0pt, mark=o, mark options={solid, red}]
  table[row sep=crcr]{%
10	105.53881113628\\
50	139.601658157338\\
90	151.839366194767\\
130	156.594354013377\\
170	163.304756847209\\
210	166.534557311289\\
250	169.578943180106\\
290	172.499867580275\\
};
\addlegendentry{w MEC}

\addplot [color=black, dashed, line width=1.0pt]
  table[row sep=crcr]{%
10	160\\
150	160\\
};

\addplot [color=black, dashed, line width=1.0pt]
  table[row sep=crcr]{%
10	255\\
150	255\\
};

\addplot [color=black, line width=1.0pt]
  table[row sep=crcr]{%
150	100\\
150	160\\
150 255\\
};

\addplot [color=red, only marks,line width=2.0pt, mark size = 5pt, mark=o, mark options={solid, green}]
  table[row sep=crcr]{%
    150	160\\
    150 255\\
};

\end{axis}

\end{tikzpicture}%
